LLM Inference Enhanced by External Knowledge: A Survey

Recent advancements in large language models (LLMs) have enhanced natural-language reasoning. However, their limited parametric memory and susceptibility to hallucination present persistent challenges for tasks requiring accurate, context-based inference. To overcome these limitations, an increasing number of studies have proposed leveraging external knowledge to enhance LLMs. This study offers a systematic exploration of strategies for using external knowledge to enhance LLMs, beginning with a taxonomy that categorizes external knowledge into unstructured and structured data. We then focus on structured knowledge, presenting distinct taxonomies for tables and knowledge graphs (KGs), detailing their integration paradigms with LLMs, and reviewing representative methods. Our comparative analysis further highlights the trade-offs among interpretability, scalability, and performance, providing insights for developing trustworthy and generalizable knowledge-enhanced LLMs.

==> contents/acknowledgement.tex <==
% \section*{Acknowledgments}



==> contents/chapter2_fig1.tex <==

\begin{figure*}[ht]
	\centering
	\resizebox{\textwidth}{!}{
		\begin{forest}
			forked edges,
			for tree={
				grow=east,
				reversed=true,
				anchor=base west,
				parent anchor=east,
				child anchor=west,
				base=center,
				font=\large,
				rectangle,
				draw=hidden-draw,
				rounded corners,
				align=left,
				text centered,
				minimum width=4em,
				edge+={darkgray, line width=1pt},
				s sep=3pt,
				inner xsep=2pt,
				inner ysep=3pt,
				line width=0.8pt,
				ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
			},
			where level=1{text width=13em,font=\normalsize,}{},
			where level=2{text width=9em,font=\normalsize,}{},
			where level=3{text width=28em,font=\normalsize,}{},
			where level=4{text width=18em,font=\normalsize,}{},
			[
				\textbf{External Knowledge Source}, ver
				[
					\textbf{Unstructured Data}  (\S \ref{sec:2_1_unstructured_data}), fill=blue!10
					[
						\textbf{Textual }(\S \ref{subsec:2_1_Textual}) , fill=blue!10
						[
							\textbf{Wikipedia, Web Pages, News, Books, Domain Documents}, fill=blue!10
						]
					]
					[
						\textbf{Non-Textual }(\S \ref{subsec:2_1_Non-Textual}) , fill=blue!10
						[
							\textbf{Images, Audio, Video}, fill=blue!10
						]
					]
				]
				[
					\textbf{Structured Data}  (\S \ref{sec:2_2_structured_data}), fill=orange!10
					[
						\textbf{Tables} (\S \ref{subsec:2_2_tables}),  fill=orange!10
                            [
                            \textbf{Spreadsheet, Web Table, Database, Document}, fill=orange!10
                            ]
					]
					[
						\textbf{KGs} (\S \ref{subsec:2_2_kgs}), fill=orange!10
                            [
                            \textbf{Wikidata, Freebase, ConceptNet, Domain-specific KGs}, fill=orange!10
                            ]
					]
				]
				
			]
		\end{forest}
        }
	\caption{Taxonomy of external knowledge source.}
	\label{fig:taxonomy_table_llm}
\end{figure*}

==> contents/chapter4.tex <==
\section{Benchmarks and Evaluation Metrics of Knowledge-Augmented LLMs}
\label{Evaluation Metrics for Knowledge-Augmented LLMs}

It is important to understand how LLMs augmented with external knowledge are assessed across diverse tasks and modalities to systematically evaluate their reasoning capabilities. This section provides an overview of widely used benchmark datasets and evaluation metrics for measuring the effectiveness of knowledge-enhanced LLM inference.

We categorize the benchmarks into three major task types, corresponding to the knowledge source utilized. \autoref{tab:evaluation-metrics} summarizes representative benchmarks along with the associated evaluation metrics for each task category, offering a structured view of how knowledge-augmented LLMs are assessed under different reasoning scenarios.

%\renewcommand{\arraystretch}{1.5}
\begin{table*}[t!]
\centering
\small
\begin{tabular}{lp{5cm} p{6.4cm}}
\toprule
\textbf{Task Type} & \textbf{Benchmarks} & \textbf{Common Evaluation Metrics} \\
\midrule
\textbf{General Knowledge QA} & 
TriviaQA, HotpotQA, FreebaseQA & Exact Match (EM), F1, Recall, BERTScore, GPT-4 Average Ranking  \\
\midrule
\textbf{Table-Based Reasoning} & 
TabFact, WikiTQ, FeTaQA, WikiSQL & 
Binary Classification Accuracy, Exact Match (EM), ROUGE \\
\midrule
\textbf{Graph-Based Reasoning} & 
WebQSP, CWQ, MetaQA & 
Hits@1, Hits@K, Path Accuracy, Entity Linking Accuracy \\
% \hline
% \textbf{Video Understanding \& QA} & 
% HowTo100M, YouCook2 & 
% BLEU, METEOR, ROUGE, VideoQA Accuracy, Temporal Reasoning Score \\
% \hline
% \textbf{Function Calling / API Interaction} & 
% ToolBench, API-Bench (if included), Gorilla & 
% Function Selection Accuracy, Argument Prediction Accuracy, Execution Success Rate \\
\bottomrule
\end{tabular}
\caption{Benchmark datasets and evaluation metrics for knowledge-augmented LLMs across various task types.}
\label{tab:evaluation-metrics}
\end{table*}


\subsection{General Knowledge Tasks}
Open-domain QA tasks evaluate a model’s ability to extract and reason over unstructured textual information, typically from sources such as Wikipedia or the open web. 
\begin{compactitem}
\item TriviaQA \cite{joshi2017triviaqa} includes trivia-style questions paired with evidence documents and primarily tests the model’s ability to retrieve and synthesize a single relevant fact. 
\item HotpotQA \cite{yang2018hotpotqa} increases task complexity by introducing multi-hop reasoning, requiring the model to aggregate information from multiple supporting documents, making it a valuable benchmark for testing whether a model can synthesize and reason across separate sources.
\item FreebaseQA \cite{jiang-etal-2019-freebaseqa} comprises factoid questions whose answers are grounded in the Freebase knowledge graph. However, since it does not provide structured queries or reasoning paths, it is typically used as an open-domain QA dataset rather than a KGQA benchmark.
\end{compactitem}

Common evaluation metrics include:
\begin{compactitem}
\item Exact Match (EM): strict string equality between predicted and ground truth answers.
\item F1 score: token-level overlap between predictions and references. 
\item Recall: particularly for retrieval coverage.
\item BERTScore: measuring semantic similarity using contextual embeddings.
\item GPT-4 Average Ranking: a preference-based metric reflecting model output quality as judged by GPT-4. 
\end{compactitem}

\subsection{Table-Based Reasoning}
\label{subsec:4_2_table}
Table reasoning tasks evaluate a model's ability to understand, retrieve, and reason over table-structured data. 
\begin{compactitem}
\item WikiTableQuestions (WikiTQ) \cite{pasupat2015compositional} is a large-scale benchmark designed to evaluate models on question answering over semi-structured tables from Wikipedia, requiring capabilities such as comparison, aggregation, and arithmetic reasoning. 
\item TabFact \cite{chen2019tabfact} is a benchmark that evaluates a model's ability to determine whether a natural language statement is entailed or refuted by tables from Wikipedia, requiring linguistic understanding and symbolic reasoning. 
\item FeTaQA \cite{nan2022fetaqa} focuses on complex reasoning and generating explanations using Wikipedia tables. 
\item WikiSQL \cite{zhong2017seq2sql} enables natural language interfaces to relational databases by translating questions into SQL queries, allowing users to access data without explicit knowledge of SQL.
\end{compactitem}

Common evaluation metrics include:
\begin{compactitem}
\item Binary Classification Accuracy: for fact verification tasks
\item Exact Match (EM): applied in table-based QA for precise string matching. 
\item ROUGE: measures n-gram overlap between generated and reference textual explanations.
\end{compactitem}

% \QianHuiComment{WikiTableQuestions (WikiTQ) \cite{pasupat2015compositional} is a large-scale dataset that challenges models to answer questions based on semi-structured tables from Wikipedia, testing tasks like comparison, aggregation, and arithmetic.
% TabFact \citep{chen2019tabfact} asks models to determine if a statement is supported or contradicted by table data, requiring both linguistic and symbolic reasoning.
% Unlike traditional QA datasets with short, fact-based answers, FeTaQA \cite{nan2022fetaqa} focuses on complex reasoning and explanation generation over Wikipedia tables, including 'what', 'how', and 'why' questions.
% WikiSQL \cite{zhong2017seq2sql} allows natural language interfaces for relational databases, converting questions into SQL queries for easier data querying without SQL knowledge.}

\subsection{Graph-Based Reasoning}
\label{subsec:4_3_kg}
Graph-based reasoning benchmarks assess a model’s ability to perform structured inference using KGs. These tasks emphasize multi-hop, entity-centric, and relation-aware reasoning.
\begin{compactitem}
\item WebQSP \cite{yih2016value} is a widely used benchmark for semantic parsing into SPARQL queries, testing both single-hop and multi-hop reasoning over entity relationships. It evaluates models for converting complex questions into executable formal logic.
\item ComplexWebQuestions (CWQ) \cite{talmor2018web} extends WebQuestions \cite{berant2013semantic} with compositional and conjunctive questions requiring integration of multiple KG facts from web snippets. It tests models on combining KG reasoning with retrieval-based evidence, making it valuable for evaluating hybrid reasoning that bridges symbolic and textual knowledge.
\item MetaQA \cite{puerto-etal-2023-metaqa} tests multi-hop KGQA using movie-related triples, covering 1-hop, 2-hop, and 3-hop queries.
\end{compactitem}

Common evaluation metrics include:
\begin{compactitem}
\item Hits@1, Hits@K: Common evaluation metrics include Hits@1 and Hits@K for assessing the proportion of correct entities ranked within the top positions.
\item Path Accuracy: for evaluating the correctness of inferred reasoning paths.
\item Entity Linking Accuracy: for measuring the precision of entity disambiguation.

\end{compactitem}

